Benchmarking Procedural Language Understanding for Low-Resource Languages: A Case Study on Turkish

Understanding procedural natural language (e.g., step-by-step instructions) is a crucial step to execution and planning. However, while there are ample corpora and downstream tasks available in English, the field lacks such resources for most languages. To address this gap, we conduct a case study on Turkish procedural texts. We first expand the number of tutorials in Turkish wikiHow from 2,000 to 52,000 using automated translation tools, where the translation quality and loyalty to the original meaning are validated by a team of experts on a random set. Then, we generate several downstream tasks on the corpus, such as linking actions, goal inference, and summarization. To tackle these tasks, we implement strong baseline models via fine-tuning large language-specific models such as TR-BART and BERTurk, as well as multilingual models such as mBART, mT5, and XLM. We find that language-specific models consistently outperform their multilingual models by a significant margin across most procedural language understanding (PLU) tasks. We release our corpus, downstream tasks and the baseline models with https://github.com/ GGLAB-KU/turkish-plu.

==> sections/dataset.tex <==
    
    
    
    %\subsection{Dataset Creation}
        %Our dataset creation process consists of three parts: i) scraping the Turkish wikiHow, ii) translating the English tutorials from the English wikiHow corpus, and iii) filtering. We obtain the Turkish wikiHow corpus by merging the filtered versions of the translated English wikiHow tutorials and the Turkish wikihow tutorials.
        %\subsubsection{Scraping Turkish Wikihow}
            %Using the beautifulsoup library \citep{richardson2007beautiful}, we scrape the Turkish wikiHow tutorials from the wikiHow's sitemap files. After the category filtering and deduplication process, we get over two thousand tutorials.
        %\subsubsection{Translating English Wikihow}
            %To translate the tutorials from the English wikiHow corpus, we develop a free open-source file-level translation tool, ÇeVeri (the conjunction of the Turkish words Çeviri, meaning translation, and Veri, meaning data). ÇeVeri is basically a Google Translate API wrapper that utilizes recursive search to find the texts within a file to translate and replace them. After filtering the English wikiHow corpus by category, we translate the remaining tutorials using ÇeVeri. This way, we obtain over fifty thousand tutorials. Please see Appendix \ref{sec:ceveri} for the details of ÇeVeri.
        %\subsubsection{Filtering}
            %We only leave the how-to tutorials from the following categories: Cars and Other Vehicles, Computers and Electronics, Health, Hobbies and Crafts, Home and Garden, Pets and Animals. The reason behind our selection of particular categories is that we want to have instructional tutorials without any personal factors within them. For example, categories such as Relationships or Youth might have specific privy cases where common sense cannot be applied. The final version of our corpus contains over 52k tutorials, +2k of which comes from the Turkish wikiHow tutorials and +50k of which comes from the translated English wikiHow tutorials.
    
    %\subsection{Machine Translation Quality Control}
    %We scrape and translate the English versions of already-existing Turkish wikiHow tutorials in order to measure the quality of machine translation done with ÇeVeri. Table \ref{table:mtqt} shows the BLEU \citep{papineni2002bleu}, ROUGE \citep{lin-2004-rouge}, and METEOR \citep{banerjee-lavie-2005-meteor} scores found.
    
    
    %\subsection{Dataset Statistics}
        
%Lastly, we derive the subgroups of task-specific data from our corpus to use in each task, which can be seen in Table \ref{table:task_specific_data}.


        
    %\subsection{Task-Specific Data}
    %\label{subsection:task_specific_data}
        %While the Turkish wikiHow corpus constitutes an umbrella dataset, we also create sub-groups of data for each procedural task we discussed in Section \ref{section:tasks}.
        %\subsubsection{Linking Actions}
        %\label{subsubsection:task_specific_data_linking_actions}
         %   In our Turkish wikiHow corpus, there are more than 1500 steps that are matched with other tutorials in the corpus. These steps are matched with other tutorials with a hyperlink redirecting them to the matched tutorials set by the editors, as an example seen in the Figure \ref{figure:step_with_a_hyperlink}. We use these steps and the goals of the matched tutorials as the ground-truth data for the linking actions task.

          %  \begin{figure}[h]
           % \centering
            %\includegraphics[width=0.5\textwidth]{Images/step_with_a_hyperlink.png}
            %\caption{An example step with a hyperlink redirecting it to a tutorial. (Step says "Connect your printer to your computer." and the redirected tutorial has the title of "How to Connect a Printer to a Computer?")}
            %\label{figure:step_with_a_hyperlink}
            %\end{figure}

        %\subsubsection{Goal Inference}
        %\label{subsubsection:goal_inference}
         %   We approach the goal inference task as a multiple choice task. For instance, when the prompt step is "Kıyafetlerini sık, böylece daha hızlı kuruyacaktır. (Squeeze your clothes, they would get dry quicker this way.)" and the candidate goals are: \\
          %  A. Lavanta Nasıl Kurutulur? (How to Dry Lavender?) \\
           % B. Kıyafetler Elde Nasıl Yıkanır? (How to Hand-Wash Clothes?) \\
            %C. Kıyafetler Çabucak Nasıl Kurutulur? (How to Dry Clothes Quickly?) \\
            %D. Islak Bir iPhone Nasıl Kurutulur? (How to Dry a Wet iPhone?) \\
            % the positive candidate would be C. \\
            
            %Our data creation method mostly follows that of \citep{zhang-etal-2020-reasoning}. We collect the prompt steps and the positive goal candidates by simply picking them iteratively from the each tutorial in our corpus. For the negative candidate sampling, we value the semantic similarity with the positive candidate and the contextual plausibility for the prompt step. We map each step in our corpus  to a vector representation by taking the average of the BERT embeddings \citep{devlin-etal-2019-bert} of the verb, noun, and proper noun tokens\footnote{We conduct the POS tagging with the nlpturk library. \href{https://github.com/nlpturk/nlpturk}{https://github.com/nlpturk/nlpturk}} contrary to \citep{zhang-etal-2020-reasoning}, which only considers the verb tokens. The reason why we included the additional parts of speech is because most of the steps and goals in our corpus contains auxiliary verbs, which are commonly used in Turkish\footnote{Such auxiliary verbs are mainly etmek, eylemek, olmak, kılmak and yapmak.}, that can be used in a wide range of contexts. Although contextualized token embeddings help distinguishing the such differences to a certain extent, we observe that the incorporation of the additional parts brings a significant improvement in our negative candidate sampling strategy. Using the vector representations, we choose the top-3 goals with the highest cosine similarity to the positive candidate as the negative candidates. We utilize FAISS \citep{johnson2019billion} to compute the top-n nearest neighbours. After the positive and negative candidate sampling, we randomly reassign one of the candidates as positive and correct the labels accordingly with a probability of 0.15 to avoid model learning the sampling strategy.

            %Lastly, we apply task-specific filters, detailed in the Appendix \ref{sec:step_and_goal_inference_filters}. For the test split, we only use the human-approved examples.
        %\subsubsection{Step Inference}
        %\label{subsubsection:step_inference}
            %We approach the step inference task as a multiple choice task. For instance, when the prompt goal is "Makas Nasıl Bileylenir? (How to Whet a Scissors?)" and the candidate steps are: \\
            %A. Camı temizle. (Clean the glass/windows.) \\
            %B. Makası sil. (Wipe the scissors.) \\
            %C. Tuvaleti sil. (Wipe the toilet.) \\
            %D. Kartonu kes. (Cut the cardboard.) \\
            %the positive candidate would be B. \\

            %We follow the same steps described in the Section \ref{subsubsection:goal_inference} to sample positive and negative candidates by simply reversing the roles of the goals and the steps in the sampling process. For the test split, we only use the human-approved examples.
        %\subsubsection{Step Ordering}
            %We approach the step inference task as a multiple choice task. For instance, when the prompt goal is
            %"YouTube'da Nasıl Yorum Bırakılır? (How to Leave a Comment on Youtube?)" and the candidate steps are: \\
            %A. Bir video arayın. (Search a Video.) \\
            %B. YouTube'u açın. (Open Youtube.) \\
            %B must precede A. \\

            %For this task, we use the sampling strategy of \citep{zhang-etal-2020-reasoning}. In wikiHow, some tutorials follow an ordered set of steps, while others contain alternative steps parallel to each other. Out of the ordered portion of our corpus, which we obtain in Appendix \ref{sec:classifying_orderliness_of_the_tutorials}, we use each goal as a prompt to sample step pairs with a window size of 1, and do not include steps with other steps between them as ordered step pairs. After the initial collection, we concatenate the step pairs to label them with the finetuned classifier model which we elaborate on in Appendix \ref{sec:classifying_orderliness_of_the_tutorials}, and retain the pairs labeled as ordered. We also randomly shuffle the pairs to prevent any index biases. For the test split, we only use the human-approved examples.
            
        %\subsubsection{Next Event Prediction}
            %We approach the next event prediction task as a multiple choice task. For instance, when the prompt goal is "Sabit Disk Nasıl Çıkarılır? (How to Remove a Hard Drive?)", prompt step is "Bilgisayarın kasasını aç. (Open the Computer Case.)" and the candidate steps are: \\
            %A. Bilgisayar kasasının içinde sabit diski bul. (Locate the hard drive inside the computer.) \\
            %B. Bilgisayarının verilerini yedekle. (Back up your computer's data.) \\
            %C. Masaüstü anakartınla uyumlu bir sabit disk satın al. (Buy a hard drive that is compatible with your desktop motherboard.) \\
            %D. Windows yüklü bir masaüstü bilgisayarının olduğundan emin ol. (Make sure that you have a Windows desktop computer.) \\
            %the positive candidate would be A. \\

           % With the subgroup of our corpus labeled as ordered, we iteratively collect the prompt goals and two consecutive steps to use the prior step as the prompt step and the later step as the positive candidate. After obtaining the positive candidate, we use the same sampling strategy that we used at \ref{subsubsection:goal_inference} with a single difference. This time, we additionally take pronoun token embeddings into account in order not to break the tutorial's narrative. For the test split, we only use the human-approved examples.
        %\subsubsection{Summarization}
            %Following the data format proposed by \citep{Koupaee2018WikiHowAL} and building on the WikiLingua's \citep{ladhak-etal-2020-wikilingua} contributions to performing summarization over Turkish procedural data, we choose the abstractive text summarization as our summarization objective. In wikiHow, each step consists of a one sentence summary-like headline and a description paragraph that details the step. For the tutorials with no methods or parts, we merge the descriptions and headlines of the steps into two separate text bodies to create document-summary pairs. For the tutorials that have methods or parts within them, we do the same on the method-or-part-level. Figure \ref{figure:step_headline_and_description} shows an example step from the tutorial "Giysiden Küf Nasıl Çıkarılır? (How to Get Mold Out of Clothing?)".

            %\begin{figure}[h]
            %\centering
            %\includegraphics[width=0.5\textwidth]%{Images/step_headline_and_description.png}
            %\caption{An example step. The bolded part is the step headline and the rest is the step description.}
           % \label{figure:step_headline_and_description}
            %\end{figure}

==> sections/discussion.tex <==
    
    % Localization issues
    As we investigate the Turkish-English article pairs, we observe that some articles are localized, not directly translated. For instance, the Turkish counterpart of the tutorial titled "How to Lose 10 Pounds in 10 Days" is "10 Günde Nasıl 5 Kilo Verilir" (How to Lose 5 Kilograms in 10 Days). So when ÇeVeri translates "How to Lose 10 Pounds in 10 Days" as "10 Günde Nasıl 10 Pound Verilir", the translation quality measurement scores will not be a perfect score even though the titles boil down to the same meaning. Although this does not affect any procedural task we study, we believe localization might have a slight impact on the translation quality measurement. Since such differences do not cause a discrepancy or degenerate the meaning, we leave them as they are.

==> sections/intro.tex <==
    A procedural tutorial is a set of steps that must be done in order to achieve the tutorial's goal. For instance, in order to take care of an indoor plant, one must i) place the plant in a suitable area, ii) increase the humidity indoors, and iii) choose the correct fertilizer. This structured nature of procedural texts facilitates the acquiring of procedural data and defining procedural tasks.

    Turkish has been studied by a dedicated research community and can be considered a resource-rich language in natural language processing \citep{joshi-etal-2020-state, coltekin2022}. Furthermore, with the emerging centralized hubs for datasets, baselines, and tools, such as MUKAYESE\footnote{\href{https://mukayese.tdd.ai}{https://mukayese.tdd.ai}} \citep{safaya-etal-2022-mukayese} and Turkish Data Depository (TDD)\footnote{\href{https://tdd.ai}{https://tdd.ai}}, it has become easier to study conventional natural language processing tasks for Turkish. However, due to the late uptrend of the popularity of procedural documents\footnote{It took more than eight years for wikiHow to have over 150k articles. \href{https://www.wikihow.com/wikiHow:Statistics}{https://www.wikihow.com/wikiHow:Statistics}}, procedural data are still not widely inclusive for underrepresented languages\footnote{Although wikiHow comprises 19 languages, only two languages (English and Spanish) have more than 100k articles in parallel \citep{ladhak-etal-2020-wikilingua}.}.
    
    In this work, we survey and study several procedural tasks, which draw a significant interest in natural language processing in Turkish. As we observe a skewed distribution of the amount of procedural data available for languages, we aspire to induce studies for other underresourced and understudied languages by designing a case study for Turkish. We aim to achieve this aspiration by introducing a document-level umbrella corpus, task-specific datasets, and baseline models.

    We work on six different procedural tasks, which we discuss in detail in Section \ref{section:tasks}. With our document-level corpus, we curate task-specific datasets for each task. Using the task-specific datasets, we evaluate existing baselines, if there is any, and provide new ones. 
    
    Our overall contributions are as follows:
    \begin{itemize}
    \item An open-domain corpus for Turkish procedural and instructional documents, which forms a basis for defining and studying procedural tasks in Turkish and encourages for the same in other underresourced languages.
    \item Datasets for six different procedural tasks, which allow for investigating procedural data in Turkish from different perspectives.
    \item Baseline models for these procedural tasks, which show strong performances.
    \end{itemize}

%   \begin{table*}[]
%     \begin{tabular}{lcc}
%     Task & Metric(s) & Baseline(s) \\ \
%     Linking Actions & Recall & \begin{tabular}[c]{@{}c@{}}BERTurk\\ XLM-R\\ S-BERTurk\\ S-XLM-R\\ XLM-R-XL-Paraphrase\\ LaBSE\\ SimCSE-TR\end{tabular} \\
%     Goal Inference & \begin{tabular}[c]{@{}c@{}}Accuracy\\ F1\\ Recall\\ Precision\end{tabular} & \begin{tabular}[c]{@{}c@{}}DistilBERTurk\\ BERTurk\end{tabular}                           \\
%     Step Inference & \begin{tabular}[c]{@{}c@{}}Accuracy\\ F1\\ Recall\\ Precision\end{tabular} & \begin{tabular}[c]{@{}c@{}}DistilBERTurk\\ BERTurk\end{tabular}                           \\
%     Step Ordering  & \begin{tabular}[c]{@{}c@{}}Accuracy\\ F1\\ Recall\\ Precision\end{tabular} & \begin{tabular}[c]{@{}c@{}}DistilBERTurk\\ BERTurk\end{tabular}                           \\
%     Next Event Prediction & \begin{tabular}[c]{@{}c@{}}Accuracy\\ F1\\ Recall\\ Precision\end{tabular} & \begin{tabular}[c]{@{}c@{}}DistilBERTurk\\ BERTurk\end{tabular}                                       \\
%     Summarization & \begin{tabular}[c]{@{}c@{}}ROUGE1\\ ROUGE2\\ ROUGE-L\end{tabular}          & \begin{tabular}[c]{@{}c@{}}TRBART\\ mBART50\\ mT5\end{tabular}                                   
%     \end{tabular}
%     \caption{List of the procedural tasks we work on. We list the evaluation metrics and baselines for each task.}
%     \label{table:task_details}
%     \end{table*}


\begin{table*}
    \begin{centering}
    \scalebox{0.55}{
    \begin{tabular}{lllll}
        & \textbf{Goal Inference} & \textbf{Step Inference} & \textbf{Step Ordering} & \textbf{Next Event Prediction} \\
        \toprule
        \multirow{2}*{Prompt} & Kıyafetlerini sık, böylece daha hızlı kuruyacaktır. & Makas Nasıl Bileylenir? & YouTube’da Nasıl Yorum Bırakılır? & Sabit Disk Nasıl Çıkarılır? \textit{(How to Remove a Hard Drive)} \\ 
                              & \textit{(Squeeze your clothes, they would get dry quicker this way.)} & \textit{(How to Whet a Scissors)} & \textit{(How to Leave a Comment on Youtube)} & Bilgisayarın kasasını aç. \textit{(Open the Computer Case.)} \\
        \midrule
        \multirow{2}*{Candidate A} & Lavanta Nasıl Kurutulur? & Camı temizle. & Bir video arayın. & Bilgisayar kasasının içinde sabit diski bul. \\
        & \textit{(How to Dry Lavender)} & \textit{(Clean the glass/windows.)}  & \textit{(Search for a Video.)}  & \textit{(Locate the hard drive inside the computer.)} \\
        \multirow{2}*{Candidate B} & Kıyafetler Elde Nasıl Yıkanır? & Makası sil. & YouTube’u açın. & Bilgisayarının verilerini yedekle. \\
        & \textit{(How to Hand-Wash Clothes)} & \textit{(Wipe the scissors.)}  & \textit{(Open Youtube.)}  & \textit{(Back up your computer’s data.)} \\
        \multirow{2}*{Candidate C} & Kıyafetler Çabucak Nasıl Kurutulur? & Tuvaleti sil. & \textemdash & Masaüstü anakartınla uyumlu bir sabit disk satın al. \\
        & \textit{(How to Dry Clothes Quickly)} & \textit{(Wipe the toilet.)}  & & \textit{(Buy a hard drive compatible with your desktop motherboard.)} \\
        \multirow{2}*{Candidate D} & Islak Bir iPhone Nasıl Kurutulur? & Kartonu kes. & \textemdash & Windows yüklü bir masaüstü bilgisayarının olduğundan emin ol. \\
        & \textit{(How to Dry a Wet iPhone)} & \textit{(Cut the cardboard.)}  &  & \textit{(Make sure that you have a Windows desktop computer.)} \\
        \bottomrule
    \end{tabular}}
    \caption{Positive candidates are C, B, B, and A respectively.}
    \label{table:keyword_manipulation_examples}
    \end{centering}
\end{table*}
